Effective Demonstration Annotation for In-Context Learning via Language Model-Based Determinantal Point Process

In-context learning (ICL) is a few-shot learning paradigm that involves learning mappings through input-output pairs and appropriately applying them to new instances. Despite the remarkable ICL capabilities demonstrated by Large Language Models (LLMs), existing works are highly dependent on large-scale labeled support sets, not always feasible in practical scenarios. To refine this approach, we focus primarily on an innovative selective annotation mechanism, which precedes the standard demonstration retrieval. We introduce the Language Model-based Determinant Point Process (LM-DPP) that simultaneously considers the uncertainty and diversity of unlabeled instances for optimal selection. Consequently, this yields a subset for annotation that strikes a trade-off between the two factors. We apply LM-DPP to various language models, including GPT-J, LlaMA, and GPT-3. Experimental results on 9 NLU and 2 Generation datasets demonstrate that LM-DPP can effectively select canonical examples. Further analysis reveals that LLMs benefit most significantly from subsets that are both low uncertainty and high diversity.

==> latex/tab/old_basic.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\definecolor{Mycolor1}{HTML}{BAD8F2}
\definecolor{Mycolor2}{HTML}{DDEEFA}
\begin{table*}[t]
{
\renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{3pt}
\definecolor{Gray}{gray}{0.9}
\newcolumntype{a}{>{\columncolor{Gray}}c}
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{lcc|c|ccccc|cc|ccc|c|a}
% \hline
\toprule
\textbf{Model}     & \textbf{Budget}                                      & \textbf{Method}   &  \textbf{SST-5}
& \textbf{RTE} & \textbf{\text{MNLI}} & \textbf{MRPC} &\textbf{BoolQ} & \textbf{QNLI}         & \textbf{TREC} & \textbf{DBpedia} &  \textbf{Hellaswag} & \textbf{\text{COPA}} & \textbf{\text{CosmosQA}} & \textbf{\text{Subj}} & \multicolumn{1}{c}{\textbf{\text{Avg.}}} \\ 
\midrule
\multirow{16}{*}{\makecell{\textsc{\textbf{GPT-J}}\\\textsc{\textbf{6B}}}}        & \multirow{8}{*}{$|\mathcal{L}|=16$}                   
& Random &47.56  & 48.01   &33.18        &    66.42  & 50.92   & 51.20    & 68.10  & 82.73   &   64.93   &  82.30 & 24.54 & 80.10
 & 58.33\\
                             &         
& MFL &37.65  & 46.20   &39.73        &    53.68  & 42.72   & 51.25    & 68.60  & 87.85   &   65.18   &  \textbf{83.00} & 24.09 & 92.05
& 57.67\\
                             &  
& Perplexity &40.32  & 48.38   &39.13        &   64.46  & 51.16   & 48.60    & 60.40  & 77.18   &   64.60   &  82.40 & 33.10 & 76.95 & 57.22
\\
                             &
& K-means &45.52  & 52.71   &\textbf{41.48}        &    47.06  & 46.12   & 52.00    & \textbf{81.20}  & \textbf{90.85}   &   65.13   &  82.36 & 30.22 & 85.15 & 59.98
\\
                             &
& Fast Vote-k &41.27  & 48.01   &37.38        &    50.98  & 45.26   & 51.13    & 67.60 & 89.73	& 65.65 &	82.60  &	28.41 &	\textbf{93.00} & 58.42
\\
                             &
& Vote-k & 41.58 &  47.29  &37.48    &   48.28  & 45.57    &  51.10      &   76.60  & 89.73 &	\textbf{66.18} &	82.20 &	27.17 &	92.95 & 58.84\\
                             &                                           
& \colorbox{Mycolor2}{LM-DPP (ours)}   &\textbf{48.69}  &  \textbf{54.67} &40.70   &   \textbf{69.12}    & \textbf{58.29}  &   \textbf{52.28}      &   68.40 &  86.25 &	65.55 &	82.40 &	\textbf{42.01} &	88.20 & \textbf{63.05}\\ 
\cmidrule{2-16} 
                             & \multirow{8}{*}{$|\mathcal{L}|=100$}     
& Random &45.20	&48.38&	38.48&	65.69&	50.12&	51.70&	74.60&	90.50&	66.03&	83.00 &	30.99 &	88.65 & 61.11\\
                             &                                          
& MFL &44.80 &	44.40 &	36.98 &	59.56 &	53.36 &	51.28 &	78.20 &	90.65 &	65.35	& 83.20 &	32.93 &	92.65 & 61.11\\
&                                          
& Perplexity &48.05 &	48.38 &	39.18 &	66.67 &	48.23 &	51.05 &	73.60 &	77.93	&64.53 &	82.20 &	31.62 &	87.90 & 59.95\\
&                                          
& K-means &44.89 &	48.74 &	40.78 &	68.14 &	50.57 &	51.78 &	73.60 &	\textbf{91.88}	&65.45 &	82.80 &	33.24 &	91.30 & 61.93\\
&                                          
& Fast Vote-k &45.61 &	48.74 &	40.15 &	64.46 &	49.14 &	51.65 &	74.40 &	91.00	& 65.50 &	83.40 &	30.79 &	\textbf{93.10} & 61.50\\
&                                          
& Vote-k &43.03 &	47.65 &	38.78 &	66.42 &	47.13 &	51.70 &	\textbf{83.00} &	87.53	& 65.70 &	82.00 &	\textbf{35.71} &	91.35 & 61.67\\
                             &                                           
& \colorbox{Mycolor2}{LM-DPP (ours)}  & \textbf{50.04} &	\textbf{54.87} &	\textbf{41.90} &	\textbf{68.38} &	\textbf{52.29}	& \textbf{52.88} & 	78.60 &	91.45 &	\textbf{66.30} &	\textbf{84.40} & 	33.87 &	92.63 & \textbf{63.97}\\
% \cmidrule{1-12}
\midrule
\multirow{16}{*}{\makecell{\textsc{\textbf{LlaMA-2}}\\\textsc{\textbf{7B}}}} & \multirow{8}{*}{$|\mathcal{L}|=16$}                    
& Random &48.91 &	\textbf{61.37} &	33.30 &	66.67 &	65.17 &	52.85 &	72.20 &	82.35	& 74.78 &	86.00 &	42.24 &	77.45 & 63.61\\
                             &                                           
& MFL &49.91 &	53.07 &	40.65 &	53.43 &	68.65 &	53.00&	78.20 &	86.08 &	\textbf{75.90}&	86.80 &	32.66 &	\textbf{91.20}& 64.13\\
&                                           
& Perplexity &47.19 &	58.12 &	38.58 &	62.75 &	\textbf{69.39} &	49.00 &	79.80 &	78.63	 &73.03 &	87.00 &	40.07 &	 81.00 & 63.71\\
&                                           
& K-means &49.77 &	52.71 & 37.88 &	52.21 &	66.36 &	53.30 &	77.00 &	\textbf{92.08}&	75.65 &	86.00 &	38.22 &	85.15 & 63.86\\
&                                           
& Fast Vote-k &51.22 &	51.62 &	41.73 &	62.25 &	68.81 &	53.28 &	78.80 &	84.50 	& 75.78 &	\textbf{87.80} &	38.09 &	91.00 & 65.41\\
&                                           
& Vote-k &\textbf{54.25} &	54.15 &	38.15 &	59.31 &	68.47 &	53.43 &	79.60 &	84.75&	75.75 &	87.20 &	37.82 &	89.20 & 65.17\\
                             &                                          
& \colorbox{Mycolor2}{LM-DPP (ours)}  & 53.12 & 55.60 &	\textbf{42.03} &	\textbf{68.14} &	66.91	& \textbf{53.50} &	\textbf{80.20} &	88.35 &	75.68 &	87.40 &	\textbf{44.79} &	89.65 & \textbf{67.11}\\ 
\cmidrule{2-16} 
                             & \multicolumn{1}{l}{\multirow{8}{*}{$|\mathcal{L}|=100$}} 
& Random &49.22 &	54.12 &	\textbf{44.53} &	64.45 &	66.51 &	51.35 &	82.20 &	93.31	& 76.95 &	86.00 &	38.02 &	88.40 & 66.26\\
                             &                   
& MFL & 54.16 &	53.43 &	38.35 &	65.20 &	\textbf{68.87} &	\textbf{54.03} &	84.20 &	93.75 &	76.00	& 87.40  &	37.62 &	91.60 & 67.05\\
&                                           
& Perplexity & 53.17 & \textbf{58.84} &	41.47 &	67.16 &	68.72 &	49.80 &	77.60 &	79.88&	73.45 &	86.20 &	37.82 &	87.35 & 65.12\\
&                                           
& K-means &49.55 &	48.74 &	40.78 &	69.12 &	65.41 & 53.48 &	\textbf{85.80} &	94.78	& 76.70 &	84.40 &	40.47 &	91.10 & 66.69\\
&                                           
& Fast Vote-k &49.22 &	55.96 &	39.45 &	\textbf{69.53} &	68.10 &	52.88 &	84.00 &	93.75	& 76.43 &	86.40 &	38.66 &	92.35 & 67.23\\
&                                           
& Vote-k &53.67 &	57.04 &	41.13 &	64.22 &	67.74 &	53.63 &	83.80 &	92.78	& 74.85 &	85.40 &	40.74 &	92.15 & 67.26\\
                             & 
& \colorbox{Mycolor2}{LM-DPP (ours)} & \textbf{54.66} &	58.12 &	42.58 &	68.87 &	67.89	& 53.13 &	84.60 &	\textbf{94.98} &	\textbf{78.13} &	\textbf{89.40} & 	\textbf{41.27} &	\textbf{92.85} & \textbf{68.87}\\ 
\bottomrule
\end{tabular}
}
}
\caption{Results with GPT-J and LlaMA-2-7B. We compare various selective annotation methods with $\{100, 16\}$ annotated examples. Bold numbers indicate the highest accuracy among all methods. Overall, the proposed method, LM-DPP, consistently outperforms across different scenarios.}
\label{tab:main_table}
\end{table*}


==> latex/tab/recency_bias.tex <==
% dbpedia Acc is 24.61 下降5.63%
% trec Acc is 0.22580645161290322 下降11.45%
% hellaswag Acc is 0.2916666666666667 下降0.03%
% copa Acc is 0.5625 下降1.18%
% mnli Acc is 0.36 下降3.15%
% qnli Acc is 0.5 上升0.3%

\begin{table}[htbp]
\def\arraystretch{1.4}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule[1.2pt]        
& MNLI & MRPC & QNLI & CosmosQA & BoolQ \\ \hline
$\text{Random}_{\text{ascending}}$ &\textbf{41.41} & 60.55 & \textbf{51.70} & 30.99 & \textbf{50.12} \\
$\text{Random}_{\text{descending}}\dagger$ & 38.48 & 65.69 & 51.45 & 32.22 & 49.48 \\
$\text{LM-DPP}_{\text{ascending}}$ & 41.63 & 67.95 & 52.73 & \textbf{34.97} & \textbf{52.81} \\
$\text{LM-DPP}_{\text{descending}}\dagger$ & 41.90 & 68.38 & 52.88 & 33.87 & 52.29 \\

\bottomrule[1.2pt]
\end{tabular}
% \vspace{-1.45cm}
}
\caption{$\dagger$ numbers are taken from Table \ref{tab:main_table}. Results with improvements in ascending order are highlighted in bold.
% We use WN18RR and FB15k-237 in inductive setting (see text for more details). 
% Following \protect\cite{inductive} we choose baseline models as BERT for Link Prediction (BLP) followed by the employed relational model (e.g. BLP-TransE) and BERT-based (BE) as the encoder for textual models.
}
\label{tab:recency}%
\end{table}
